Graph integration of structured, semistructured and unstructured data for data journalism

Digital data is a gold mine for modern journalism. However, datasets which interest journalists are extremely heterogeneous, ranging from highly structured (relational databases), semi-structured (JSON, XML, HTML), graphs (e.g., RDF), and text. Journalists (and other classes of users lacking advanced IT expertise, such as most non-governmental-organizations, or small public administrations) need to be able to make sense of such heterogeneous corpora, even if they lack the ability to define and deploy custom extract-transform-load workflows, especially for dynamically varying sets of data sources. We describe a complete approach for integrating dynamic sets of heterogeneous datasets along the lines described above: the challenges we faced to make such graphs useful, allow their integration to scale, and the solutions we proposed for these problems. Our approach is implemented within the ConnectionLens system; we validate it through a set of experiments.

==> images/edge-specif-tikz.tex <==
\tikzstyle{arrow} = [thick,->,>=stealth]
\begin{tikzpicture}[node distance=1.3cm]
\node (zero) {$~$};
\node (n1) [right of=zero, xshift=-13mm, shape=circle, draw=black] {$n_1$};
\node (c1) [above of=n1, yshift=-8mm] {$es_1$}; 
\node (x) [right of=n1, xshift=8mm] {$x$}; 
\node (n2) [right of=n1, xshift=39mm] {$n_2$};
\draw [arrow, color=blue]  (x) -> (n1) node [midway, fill=white] {\textcolor{blue}{$l$}};
\node (dots1) [right of=n1, xshift=6mm, yshift=6mm] {$\ldots$};
\draw [arrow, color=blue]  (dots1) -> (n1) node [midway, fill=white] {\textcolor{blue}{$l$}};
\node (dots2) [right of=n1, xshift=6mm, yshift=-6mm] {$\ldots$};
\draw [arrow, color=blue]  (dots2) -> (n1) node [midway, fill=white] {\textcolor{blue}{$l$}};
\node (dots3) [left of=n2, , xshift=-6mm,yshift=6mm] {$\ldots$};
\draw [arrow, color=violet]  (dots3) -> (n2) node [midway, fill=white] {\textcolor{violet}{$l$}};
\node (dots4) [left of=n1, yshift=6mm] {$\ldots$};
\draw [arrow]  (n1) -> (dots4) node [midway, fill=white] {$b$};
\node (dots5) [left of=n1, yshift=-6mm] {$\ldots$};
\draw [arrow]  (dots5) -> (n1) node [midway, fill=white] {$c$};
\node (dots6) [right of=n2, yshift=6mm] {$\ldots$};
\draw [arrow]  (dots6) -> (n2) node [midway, fill=white] {$d$};
\node (dots7) [left of=n2, xshift=-6mm, yshift=-6mm] {$\ldots$};
\draw [arrow, color=violet]  (dots7) -> (n2) node [midway, fill=white] {\textcolor{violet}{$l$}};
\end{tikzpicture}
